Diameters of Open Star Clusters

The present paper presents a tabulation of data on all 600 Galactic open clusters for which it is presently possible to calculate linear diameters. As expected, the youngest `clusters' with ages < 15 Myr, contain a significant (greater than or equal to 20%) admixture of associations. Among intermediate-age clusters, with ages in the range 15 Myr to 1.5 Gyr, the median cluster diameter is found to increase with age. Small compact clusters are rare among objects with ages > 1.5 Gyr. Open clusters with ages > 1 Gyr appear to form what might be termed a `cluster thick disk', part of which consistst of objects that were probably captured gravitationally by the main body of the Galaxy.

==> sidneytab1.tex <==

                             TABLE 1

                    DIAMETERS OF OPEN CLUSTERS

No.   Name       l   D(pc) R(pc) Z(pc) E(B-V) log T

001 Trumpler 31 002  1.43   986  -0039  0.35  8.87
002 N6520       002  2.29  1577  -0078  0.43  7.72
003 N6530       006  5.42  1330  -0031  0.33  6.87
004 Bochum 14   006  0.34   578  -0005  1.51  7.00
005 N6514       007  6.65   816  -0004  0.19  7.37
006 N6546       007  3.82   938  -0023  0.49  7.85
007 N6531       007  2.91  1205  -0007  0.28  7.07
008 N6494       009  5.30   628  +0031  0.36  8.48
009 Markar. 38  011  0.86  1471  -0024  0.40  6.88
010 Trumpler 33 012  2.55  1755  -0099  0.36  7.68
011 Collin. 469 012  1.29  1481  -0020  0.42  7.80
012 N6603       012  6.28  3600  -0082  0.79  8.30
013 I4725       013  5.23   620  -0048  0.48  7.96
014 N6613       014  1.88  1296  -0023  0.45  7.22
015 Collin. 394 014  4.42   690  -0112  0.24  7.80
016 N6618       015  9.45  1300  -0017  1.51  6.00
017 N6716       015  2.30   789  -0131  0.22  7.96
018 Blanco 1    015  5.48   269  -0264  0.01  7.80
019 N6611       016  3.05  1749  +0024  0.78  6.88
020 Trumpler 32 017  2.50  1720  +0039  0.64  8.48
021 N6604       018  2.47  1696  +0050  0.97  6.81
022 N6631       019  4.54  2600  -0008  0.45  8.60
023 Rupr. 147   021  1.27   174  -0039  0.15  ...
024 N6649       021  1.99  1369  -0019  1.20  7.57
025 N6694       023  3.26  1600  -0081  0.59  7.93
026 N6664       024  4.06  1164  -0006  0.71  7.16
027 N6683       026  1.04  1197  -0016  0.54  7.00
028 N6705       027  7.10  1877  -0091  0.43  8.30
029 Basel 1     027  3.17  2178  -0074  0.48  7.89
030 N6704       028  4.33  2974  -0115  0.72  7.86
031 Trumpler 35 028  1.75  1206  +0000  1.22  7.86
032 Collin. 359 029 17.37   249  +0054  0.19  7.51
033 I4665       030  7.17   352  +0103  0.17  7.63
034 Berkeley 79 031  4.01  2300  +0033  1.19  7.81
035 Alessi 10   031  2.69   513  -0184  0.22  8.35
036 Berkeley 81 033  4.36  3000  -0131  1.00  9.00
037 N6994       035  1.62   620  -0346  0.07  9.40
038 N6633       036  2.19   376  +0054  0.18  8.63
039 Berkeley 42 036  2.66  1826  -0069  0.76  9.32
040 I4756       036  5.49   484  +0044  0.19  8.70
041 N6755       038  5.79  1421  -0042  0.83  7.72
042 N6756       039  1.75  1507  -0044  1.18  7.79
043 Alessi 19   040 14.08   550  +0121  0.04  8.00
044 N6709       042  4.38  1075  +0088  0.30  8.18
045 Berkeley 82 046  0.50   860  +0024  1.02  7.49
046 Collin. 399 054 33.42  1291  +0044  0.38  8.20
047 N6802       055  1.63  1124  +0018  0.85  8.87
048 Harvard 20  056  3.14  1540  -0125  0.25  7.48
049 Roslund 3   058  2.13  1467  -0120  0.35  8.04
050 N6823       059  3.30  1893  -0005  0.84  6.82
051 N6830       060  2.38  1639  -0051  0.50  7.57
052 Stock 1     060  7.45   320  +0013  0.15  ...
053 Turner 1    063  1.95  1675  +0021  0.48  7.46
054 N7036       064  1.16  1000  -0366  0.10  9.50
055 N6885       065  1.74   597  -0042  0.08  9.16
056 N6834       065  3.01  2067  +0043  0.71  7.88
057 Stephen. 1  066  2.27   390  +0104  0.04  7.73
058 Roslund 4   066  2.65  2510  -0056  0.99  7.45
059 Alessi 12   067  6.25   537  -0107  0.08  8.10
060 Saurer 6    067  4.89  9330  +0511  0.77  9.29
061 N6940       069  5.60   770  -0096  0.21  8.86
062 N6791       069 17.03  5853  +1107  0.12  9.64
063 Roslund 5   071  5.66   389  +0002  0.10  7.83
064 N6871       072 13.28  1574  +0056  0.44  6.96
065 Biurakan 2  072  6.43  1106  +0026  0.36  7.01
066 N6819       073  3.43  2360  +0348  0.24  9.17
067 Basel 6     074  3.15  1548  +0089  0.58  7.98
068 I4996       075  3.02  1732  +0039  0.67  6.95
069 Berkeley 87 075  1.84   633  +0003  1.37  7.15
070 Dolidze 42  076  1.98   972  +0018  0.57  7.54
071 Berkeley 86 076  1.94  1112  +0025  0.90  7.12
072 N6913       076  3.34  1148  +0012  0.74  7.11
073 I1311       077  7.76  5333  +0398  0.76  8.62
074 N6910       078  3.31  1139  +0040  0.97  7.13
075 N6811       079  4.95  1215  +0253  0.16  8.80
076 N6866       079  5.91  1450  +0173  0.17  8.58
077 N7063       083  1.80   689  -0118  0.09  7.98
078 Berkeley 54 083  2.68  2300  -0166  0.77  9.60
079 N7044       085  5.52  3161  -0229  0.59  9.28
080 N6996       086  1.44   620  +0001  0.54  8.00
081 N7039       087  3.87   951  -0028  0.13  7.82
082 Basel 12    088  1.71  1466  -0032  0.57  8.50
083 Basel 14    088  1.40   964  -0060  0.65  8.30
084 Basel 13    088  3.60  1236  -0027  0.34  8.80
085 I1369       089  3.03  2083  -0015  0.57  8.64
086 N7062       089  2.15  1480  -0071  0.45  8.46
087 Basel 15    090  2.36  1355  -0002  0.67  8.50
088 N7082       091 10.49  1442  -0073  0.24  8.23
089 N7067       091  1.16  1332  -0039  0.85  7.49
090 N7031       091  3.67   900  +0036  0.85  8.14
091 N7092       092  2.75   326  -0013  0.01  8.44
092 Platais 1   092  3.69  1268  -0036  0.36  8.24
093 I5146       094  4.96   852  -0082  0.59  8.02
094 N7086       094  4.53  1298  +0005  0.81  8.14
095 N7209       095  4.76  1168  -0149  0.17  8.62
096 N6939       095  3.45  1185  +0253  0.32  9.35
097 N7128       097  2.68  2307  +0017  1.02  7.25
098 N7243       098  6.82   808  -0078  0.22  8.06
099 Trumpler 37 099 21.61   835  +0054  0.47  7.05
100 I1442       101  3.41  2346  -0090  0.54  6.98
101 N7245       101  3.06  2106  -0068  0.47  8.25
102 N7226       101  1.52  2616  -0027  0.54  8.44
103 N7235       102  4.11  2823  +0039  0.93  7.07
104 N7772       102  1.31  1500  -1047  0.03  9.17
105 Berkeley 94 103  2.30  2630  -0054  0.61  7.00
106 Berkeley 96 103  1.80  3087  -0111  0.63  6.82
107 N7160       104  1.15   789  +0089  0.38  7.28
108 N7261       104  2.44  1681  +0027  0.97  7.67
109 Berkeley 93 105  3.26  5600  +0713  1.50  8.00
110 N7142       105  5.89  1686  +0278  0.40  9.28
111 Pismis-M 1  106  1.57   900  +0083  ...   ...
112 N7380       107 12.93  2222  -0034  0.60  7.08
113 King 10     108  3.93  3379  -0023  1.14  7.45
114 N7419       109  2.01  1382  +0027  1.83  7.28
115 Colin. 285  109  9.90    25  +0018  0.00  8.30
116 King 19     110  2.86  1967  +0005  0.55  8.56
117 N7510       110  3.62  2075  +0002  0.86  7.58
118 Markar. 50  111  1.23  2114  -0008  0.81  7.10
119 N7654       112  6.20  1421  +0011  0.65  7.76
120 Stock 17    115  0.62  2144  +0010  0.74  6.78
121 N7789       115 16.99  2337  -0219  0.22  9.24
122 King 21     115  2.45  2103  +0025  0.89  7.16
123 Berkeley 99 115  7.13  4900  +0860  0.30  9.50
124 King 12     116  2.08  2378  -0005  0.59  7.04
125 N7788       116  2.76  2374  -0032  0.28  7.59
126 N7790       116  4.28  2944  -0052  0.53  7.75
127 Berkeley 58 116  5.40  3715  -0084  0.55  8.40
128 King 11     117  4.21  2892  +0326  1.27  9.05
129 N7762       117  3.03   744  +0076  0.71  8.42
130 Berkeley 60 118  3.81  4365  -0125  0.86  8.20
131 Berkeley 2  119  3.05  5250  -0211  0.80  8.90
132 N103        119  3.52  3026  -0073  0.41  8.13
133 N129        120  8.98  1625  -0072  0.55  7.89
134 N136        120  1.79  4093  -0091  0.56  8.30
135 N133        120  1.28   630  +0006  0.60  7.00
136 King 14     120  4.53  2593  +0017  0.41  7.92
137 King 15     120  2.76  3162  -0051  0.70  8.40
138 N146        120  6.17  3032  +0027  0.48  7.82
139 N189        121  0.66   752  -0023  0.42  7.00
140 Stock 24    121  4.10  2818  -0044  0.50  8.08
141 N225        122  2.29   657  -0012  0.27  8.11
142 N188        122 10.12  2047  +0780  0.08  9.63
143 King 2      122  8.36  5750  -0470  0.31  9.78
144 I1590       123 24.80  2940  -0320  0.32  6.54
145 Alessi 1    123  4.22   302  -0069  0.09  8.20
146 Berkeley 62 123  2.67  1837  +0035  0.85  7.18
147 N366        124  1.82  1785  -0018  1.26  7.41
148 N381        124  2.00  1148  -0024  0.40  8.50
149 N433        125  1.35  2323  -0106  0.86  7.50
150 N436        126  4.38  3014  -0205  0.46  7.93
151 N457        126 14.13  2429  -0186  0.47  7.32
152 N559        127  2.20  1258  +0016  0.79  7.75
153 Colind.463  127  5.92   702  +0117  0.26  8.37
154 N609        127  3.47  3981  +0145  0.35  9.23
155 N581        128  3.19  2194  -0069  0.38  7.34
156 Trumpler 1  128  2.24  2563  -0051  0.58  7.48
157 Platais 2   128 19.61   201  -0102   ...  8.60
158 N637        128  1.88  2160  +0065  0.63  6.98
159 N654        129  2.97  2041  -0013  0.87  7.15
160 N659        129  2.82  1938  -0053  0.65  7.55
161 N663        129  7.95  1952  -0032  0.78  7.21
162 I166        130  8.08  3970  -0013  1.05  8.63
163 Berkeley 7  130  2.99  2570  +0017  0.80  6.60
164 Berkeley 64 131  2.32  3981  +0320  1.05  9.00
165 N744        132  1.76  1207  -0130  0.38  8.25
166 Stock 2     133  3.97   303  -0010  0.38  8.23
167 Basel 10    134  1.13  1944  -0089  0.77  7.61
168 N869        134 10.89  2079  -0136  0.58  7.07
169 Stock 7     134  1.02   698  +0000  0.61  7.21
170 I1805       134 10.97  1886  +0030  0.82  6.82
171 N884        135 12.28  2345  -0146  0.56  7.03
172 Czernik 13  135  4.61  3961  +0160  0.76  6.85
173 N1027       135  4.49   772  +0021  0.32  8.20
174 Czernik 8   135  0.82  1409  -0039  0.80  7.90
175 Berkeley 65 135  3.31  2274  +0011  1.12  7.00
176 King 4      136  4.61  3172  -0066  0.86  7.60
177 N957        136  5.28  1815  -0084  0.84  7.04
178 N752        137  9.97   457  -0180  0.03  9.05
179 I1848       137 10.48  2002  +0032  0.60  6.84
180 Trumpler 2  137  3.22   651  -0044  0.32  8.17
181 Platais 3   139 10.18   161  +0045  ...   8.60
182 Berkeley 66 139  6.05  5200  +0020  1.25  9.70
183 N1220       143  2.09  1800  -0124  0.70  7.78
184 King 6      143  2.53   871  -0001  0.50  8.34
185 N1039       143  5.08   499  -0134  0.07  8.25
186 N1502       143  1.91   821  +0109  0.76  7.05
187 King 5      143  2.76  1900  -0142  ...   9.00
188 N1245       146  7.53  2876  -0446  0.30  8.70
189 N1193       146  3.75  4300  -0909  0.12  9.90
190 Melotte 20  146 16.12   185  -0023  0.09  7.85
191 I361        147  1.87  1070  +0106  1.12  7.72
192 N1444       148  1.40  1199  -0027  0.71  7.96
193 King 7      149  4.48  2200  -0039  1.25  8.80
194 N1496       149  1.43  1230  +0004  0.45  8.80
195 Waterloo 1  151  6.40  4400  +0137  0.90  ...
196 N1528       152  3.61   776  +0003  0.26  8.57
197 Alessi 2    152  4.37   501  +0055  0.18  8.50
198 N1513       152  3.84  1320  -0036  0.67  8.11
199 N1545       153  3.72   711  +0002  0.30  8.45
200 N1342       154  2.90   665  -0176  0.32  8.66
201 Berkeley 11 157  4.19  2881  -0183  0.95  7.72
202 N1605       158  4.47  2552  -0071  0.97  7.61
203 Rupr. 148   160  3.52  3028  -0021  0.70  7.72
204 I348        160  0.78   385  -0117  0.93  7.64
205 Berkeley 12 161  3.68  3162  -0110  0.70  9.67
206 N1664       161  3.14  1199  -0009  0.25  8.46
207 Berkeley 69 162  5.86  1678  -0070  0.67  8.39
208 Berkeley 14 162  8.00  5500  +0068  0.52  9.20
209 Berkeley 18 163 20.25  5800  +0507  0.46  9.63
210 Melotte 22  166  5.23   150  -0060  0.03  8.13
211 Berkeley 70 166  7.26  4158  +0260  0.48  9.67
212 Czernik 20  168  3.92  3370  +0078  0.42  7.17
213 Waterloo 2  168  0.66   570  +0031  0.17  ...
214 N1778       168  3.42  1469  -0052  0.34  8.16
215 Stock 10    171  2.76   380  +0024  0.06  8.35
216 N1912       172  6.20  1066  +0013  0.25  8.46
217 N1907       172  3.17  1556  +0008  0.42  8.57
218 Stock 8     173  7.42  1821  -0009  0.44  7.06
219 N1893       173 10.50  3280  -0096  0.58  7.03
220 N1931       173  4.49  3086  +0015  0.74  7.00
221 Berkeley 69 174  2.50  2860  -0089  0.65  8.95
222 N1960       174  3.83  1318  +0025  0.22  7.47
223 N2281       174  4.06   558  +0162  0.06  8.55
224 Berkeley 17 175  5.50  2700  -0172  0.70 10.08
225 King 8      176  7.45  6403  +0346  0.58  8.62
226 Berkeley 19 176  5.62  4831  -0302  0.40  9.49
227 N2099       177  5.63  1383  +0075  0.30  8.54
228 N1758       179  1.99   760  -0138  0.34  8.60
229 N1750       179  3.67   630  -0117  0.34  8.30
230 Basel 4     179  8.25  5675  +0119  0.53  7.00
231 Melotte 25  180  4.31    45  -0017  0.01  8.90
232 N1647       180  6.28   540  -0156  0.37  8.16
233 Platais 4   180 16.37   276  -0052  ...   8.00
234 N1817       186  9.18  1972  -0447  0.33  8.61
235 I2157       186  2.97  2040  +0045  0.55  7.80
236 N2129       186  2.20  1515  +0001  0.65  7.32
237 Kharchen. 1 186  5.13  2520  +0095  ...   ...
238 N2168       186  5.93   816  +0032  0.26  7.98
239 N2158       186  7.38  5071  +0158  0.36  9.02
240 Berkeley 21 186  7.27  5000  -0219  0.76  9.34
241 Basel 11b   187  1.48  1692  -0033  0.32  7.82
242 N1662       187  2.54   437  -0157  0.30  8.62
243 N2266       187  4.95  3400  +0608  0.10  8.80
244 N2175       190  2.37  1627  +0014  0.60  6.95
245 Berkeley 23 192  8.05  6918  +0657  0.40  8.90
246 Collind. 69 195  8.98   441  -0092  0.10  7.05
247 N2169       195  1.53  1052  -0054  0.20  7.07
248 N2304       197  3.48  3991  +0617  0.10  8.90
249 N2194       197  9.90  3781  -0155  0.38  8.52
250 Berkeley 29 197 25.95 14871  +2076  0.16  9.02
251 N2141       198 11.73  4033  -0408  0.25  9.23
252 N2420       198  4.49  3085  +1036  0.03  9.05
253 Collind.74  198  3.65  2510  -0453  0.38  9.11
254 Berkeley 22 199  2.23  7663  -1073  0.70  9.03
255 N2259       201  2.89  3311  +0120  0.59  8.50
256 Trumpler 5  202 12.22  3000  +0055  0.58  9.61
257 N2264       202  7.57   667  +0026  0.05  6.95
258 N2355       203  4.48  2200  +0450  0.12  8.85
259 Berkeley 20 203  4.89  8400  -2494  0.12  9.78
260 N2186       203  2.10  1445  -0156  0.27  7.74
261 N2251       203  3.87  1329  +0002  0.19  8.43
262 Basel 8     203 11.20  1328  -0003  0.37  8.01
263 Basel 7     203  2.45  1684  +0016  0.40  8.03
264 N2254       204  3.44  2364  +0002  0.40  8.31
265 N2236       204  5.97  2930  -0087  0.48  8.54
266 N2395       204  2.09   512  +0124  0.12  9.07
267 Collind. 70 205 15.76   387  -0115  0.04  6.98
268 Platais 6   205 25.49   348  -0038  ...   7.78
269 Collind. 97 205  4.58   630  -0019  0.00  8.00
270 N2112       205  4.45   850  -0186  0.63  9.30
271 N2632       205  3.81   187  +0100  0.01  8.86
272 Berkeley 31 206 12.03  8272  +0738  0.08  9.31
273 N2244       206 12.19  1445  -0052  0.46  6.90
274 Collind.107 207 14.66  1738  -0027  0.54  7.00
275 N2269       207  1.47  1687  +0009  0.40  8.42
276 Berkeley 32 207  5.41  3100  +0238  0.16  9.53
277 Collind. 96 207  3.36   962  -0057  0.51  7.03
278 vdBergh 1   208  2.45  1687  -0053  0.71  8.02
279 N1976       209  5.45   399  -0132  0.05  7.11
280 Collind.110 209 10.21  1950  -0067  0.50  9.15
281 Berkeley 28 210  2.23  2557  +0067  0.76  7.85
282 Berkeley 30 210  4.18  4790  +0389  0.50  8.48
283 Dolidze 25  211 36.67  6304  -0140  0.72  6.84
284 Bochum 2    212  1.16  2661  -0018  0.83  6.66
285 N2301       212  3.55   872  +0004  0.03  8.22
286 N2324       213  7.75  3805  +0219  0.13  8.63
287 Sauer 1     214 13.93 11970  +1425  0.12  9.85
288 N2232       214  4.70   359  -0046  0.03  7.73
289 N2286       215 11.80  2897  -0115  0.17  8.88
290 N2682       215  6.60   908  +0476  0.06  9.41
291 N2215       215  2.63  1293  -0227  0.30  8.37
292 N2311       217  4.00  2290  -0028  0.33  8.60
293 Bochum 3    218  2.05  1762  +0011  0.24  7.89
294 N2302       219  1.72  1182  -0064  0.21  7.85
295 N2309       219  3.65  2511  -0098  0.35  8.40
296 Melotte 111 221  3.35    96  +0095  0.01  8.65
297 N2323       221  3.78   929  -0022  0.21  8.10
298 Berkeley 39 223  9.73  4730  +0838  0.12  9.90
299 N2335       223  2.47  1417  -0029  0.39  8.21
300 N2343       224  1.54  1056  -0022  0.12  7.10
301 N2353       224  5.86  1119  +0008  0.07  7.97
302 Berkeley 33 225  5.39  4635  -0374  0.70  8.85
303 N2204       226  7.65  2629  -0729  0.08  8.90
304 N2345       226  7.86  2251  -0091  0.62  7.85
305 Haffner 8   227  1.72  1182  +0028  0.03  9.15
306 Haffner 6   227  5.33  3054  +0014  0.45  8.83
307 N2548       227  6.71   769  +0204  0.03  8.56
308 Basel 11a   228  2.21  1520  -0021  0.00  8.30
309 N2374       228  5.12  1468  +0026  0.09  8.46
310 Platais 5   228 23.71   272  -0088  ...   7.78
311 Melotte 71  228  6.42  3154  +0247  0.11  8.37
312 N2401       229  3.43  5888  +0190  0.35  7.80
313 N2360       229  7.14  1887  -0047  0.11  8.75
314 Waterloo 7  230  2.12  2800  +0030  0.42  ...
315 N2423       230  2.67   766  +0047  0.10  8.87
316 N2506       230 12.08  3460  +0597  0.08  9.04
317 Czernik 29  230  6.06  4168  +0068  0.48  8.30
318 Haffner 10  230  4.58  5248  +0092  0.52  9.10
319 N2422       230  3.56   490  +0027  0.07  7.86
320 N2287       231  7.86   693  -0126  0.03  8.38
321 N2414       231  5.03  3455  +0117  0.51  6.98
322 N2425       231  5.89  4053  +0231  0.31  9.20
323 N2437       231  8.00  1375  +0097  0.15  8.39
324 Tombaugh 1  232  4.36  3000  -0382  0.40  9.00
325 Bochum 5    232  3.80   872  +0012  0.19  7.54
326 Bochum 4    232  3.33  2291  +0031  0.63  7.00
327 Tombaugh 2  232 11.57 13260  -1588  0.08  9.01
328 N2539       233  3.57  1363  +0263  0.08  8.57
329 Bochum 6    234 11.58  3981  -0015  0.70  7.00
330 Collind.121 235 12.19   471  -0084  0.03  7.05
331 N2383       235  2.41  1655  -0071  0.21  7.17
332 N2384       235  3.08  2116  -0088  0.26  6.90
333 N2432       235  3.32  1905  +0059  0.23  8.80
334 N2367       235  2.91  2004  -0134  0.33  6.74
335 N2421       236  4.44  2181  +0003  0.45  7.37
336 Alessi 13   236 13.41   110  -0090  0.04  ...
337 N2362       238  2.02  1389  -0134  0.10  6.91
338 Trumpler 7  238  2.14  1474  -0086  0.27  7.43
339 Ruprecht 46 238  0.66   752  +0077  0.07  9.60
340 N2354       238 21.39  4085  -0483  0.31  8.13
341 N2243       239  6.48  4458  -1379  0.05  9.03
342 Ruprecht 18 239  2.15  1056  -0091  0.70  7.65
343 N2447       240  3.02  1037  +0002  0.05  8.59
344 Ruprecht 32 241  7.78  5346  -0053  0.50  7.08
345 N2482       241  3.91  1343  +0048  0.09  8.60
346 Haffner 16  242  4.60  3165  +0026  0.18  7.08
347 Ruprecht 20 242  1.76  1208  -0121  0.10  8.50
348 Waterloo 3  242  3.03  5200  +0131  0.34  ...
349 Ruprecht 36 242  2.44  1681  -0010  0.17  7.61
350 Collind.132 242 10.98   472  -0072  0.04  7.08
351 Trumpler 9  243  3.33  2289  +0051  0.25  8.00
352 Haffner 19  243  2.96  5094  +0047  0.42  6.93
353 Haffner 18  243  3.51  6028  +0047  0.61  6.89
354 N2467       243  5.52  1355  +0009  0.34  7.10
355 N2453       243  2.50  2150  -0035  0.45  7.19
356 Ruprecht 49 244  1.06  1823  +0072  0.26  7.93
357 N2483       244  3.38  1659  +0007  0.30  7.09
358 Haffner 21  244  2.58  2951  +0084  0.11  7.92
359 Collind.140 244  3.42   405  -0056  0.03  7.55
360 Ruprecht 44 245 13.76  4730  +0040  0.62  6.94
361 N2527       246  1.75   601  +0019  0.04  8.65
362 N2439       246 10.09  3855  -0300  0.41  7.25
363 N2489       246  6.91  3957  -0053  0.37  7.26
364 Haffner 20  246  2.72  3117  -0051  0.57  8.12
365 Haffner 17  247  1.68  2880  -0127  1.26  7.70
366 N2533       247  4.91  3379  +0077  0.05  8.88
367 Haffner 15  247  1.81  2078  -0151  1.14  7.17
368 Bochum 15   247  2.45  2806  -0268  0.58  6.74
369 Arp-Mado. 2 248  7.76 13341  -1366  0.57  9.34
370 Ruprecht 47 248  3.50  3006  -0010  0.28  7.89
371 Collind.135 248  4.60   316  -0061  0.03  7.41
372 N2571       249  3.12  1342  +0083  0.14  7.49
373 N2567       249  3.41  1677  +0087  0.13  8.47
374 Ruprecht 55 250  7.12  4892  +0069  0.56  6.85
375 N2627       251  4.73  2034  +0236  0.09  8.57
376 N2451B      252  9.49   302  -0035  0.06  7.65
377 N2588       252  2.29  5248  +0224  0.30  8.60
378 Ruprecht 59 253  0.76   874  +0014  0.09  7.73
379 N2477       253  5.33  1222  -0124  0.28  8.85
380 BH 23       254  4.96   437  -0007  0.06  7.10
381 N2658       254  3.53  2021  +0214  0.04  9.15
382 N2579       254  2.10  1033  +0004  0.15  7.61
383 N2546       254 18.71   919  -0032  0.13  7.87
384 Collind.185 255  2.59  1486  +0014  0.21  8.11
385 Pismis 1    255  5.15  5907  -0073  0.58  7.93
386 N2635       255  1.67  5754  +0397  0.35  8.50
387 Pismis 3    257  2.03  1394  +0012  1.30  9.03
388 Alessi 3    257  6.03   288  -0076  0.11  8.70
389 Saurer 2    257  5.47  4700  -0082  1.24  9.40
390 Pismis 2    258  3.85  3310  -0193  0.05  9.06
391 Pismis 5    259  0.51   869  +0014  0.42  7.20
392 Rupr. 72    259  2.63  3019  +0230  0.24  9.10
393 Rupr. 158   259  2.42  4168  +0323  0.24  9.20
394 Melotte 66  259 17.56  4313  -1061  0.14  9.44
395 Collind.173 261 45.22   421  -0060  0.05  7.14
396 Collind.197 261  6.09   838  +0014  0.55  7.13
397 N2818       261  4.86  1855  +0277  0.12  8.63
398 N2671       262  2.90  1660  +0023  1.04  7.90
399 Trumpler 10 262  3.58   424  +0005  0.03  7.54
400 Ruprecht 67 262  2.62  1504  -0021  0.43  8.26
401 Pismis 4    262  4.31   593  -0025  0.01  7.53
402 N2659       264  2.49  1713  -0003  0.51  6.89
403 N2547       264  3.31   455  -0068  0.04  7.56
404 N2645       264  1.46  1668  -0085  0.38  7.28
405 Waterloo 6  264  0.92  1578  -0073  0.24  7.67
406 Pismis 8    265  1.14  1312  -0059  0.71  7.43
407 Bochum 7    265 33.48  5754  +0197  0.86  7.00
408 N2660       265  2.88  2826  -0149  0.31  9.03
409 I2395       266  3.49   705  -0044  0.07  7.22
410 Platais 9   266 20.00   174  +0010  ...   8.00
411 N2670       267  2.42  1188  -0075  0.43  7.69
412 Collind.205 269  2.70  1853  -0060  0.75  7.20
413 I2391       270  3.05   175  -0021  0.01  7.66
414 N2669       270  6.09  1046  -0111  0.18  7.93
415 Pismis 11   271  1.63  2800  -0020  1.25  7.34
416 N2866       273  1.11  1901  -0025  0.63  7.66
417 Ruprecht 76 273  1.84  1262  -0021  0.38  7.73
418 N2516       273  3.57   409  -0112  0.10  8.05
419 N1252       274  2.61   640  -0496  0.02  9.48
420 N 2972      274  1.80  2062  +0063  0.34  7.97
421 N2910       275  3.03  2607  -0054  0.34  8.20
422 Ruprecht 78 275  1.43  1641  -0054  0.35  7.99
423 N2925       275  2.25   774  -0017  0.08  7.85
424 BH 66       276  8.14  7000  -0367  0.40  8.90
425 Ruprecht 77 276  6.01  4129  -0225  0.62  7.50
426 Ruprecht 79 277  2.88  1979  -0025  0.72  7.09
427 Platais 8   277 35.94   132  -0018  ...   7.78
428 Ruprecht 82 277  3.57  2455  -0020  0.29  8.50
429 Pismis 16   277  1.06  1824  +0022  0.56  7.84
430 I2488       277  5.94  1134  -0087  0.23  8.11
431 Basel 20    277  5.89  2024  -0122  0.41  7.42
432 Ruprecht 83 278  2.15  2459  -0026  0.45  8.45
433 N1901       279  1.81   415  -0230  0.06  8.92
434 N3033       279  1.07   922  -0033  0.33  7.84
435 N3105       279  2.84  4884  +0022  0.99  7.24
436 N3228       280  0.79   544  +0043  0.03  7.93
437 BH 90       283  2.99  2572  -0066  0.53  7.94
438 N3114       283  9.27   911  -0061  0.07  8.09
439 N3330       284  1.04   894  +0060  0.05  8.23
440 Westerl. 2  284  1.09  1874  -0011  0.78  7.22
441 Trumpler 11 284  4.51  3100  -0263  0.21  ...
442 N3247       284  1.80  1547  -0009  0.22  8.08
443 I2581       284  3.56  2446  +0002  0.42  7.14
444 Saurer 3    285  6.16  8830  +0462  0.62  9.45
445 N3293       285  4.06  2327  +0003  0.26  7.01
446 Collind.223 286  4.41  1686  -0048  0.26  7.01
447 N3255       286  0.84  1445  -0066  0.25  8.30
448 N3324       286  8.09  2317  -0008  0.44  6.75
449 Carraro 1   286  2.21  1900  -0010  0.25  9.48
450 BH 99       286  2.95   507  -0006  0.06  7.60
451 N3680       286  1.36   938  +0273  0.07  9.08
452 Bochum 9    286 20.07  4600  -0126  0.63  ...
453 Bochum 10   287 11.79  2027  -0011  0.31  6.86
454 ESO 092-18  287 15.43 10607  -1229  0.50  9.02
455 Colind. 228 287  8.96  2201  -0039  0.34  6.83
456 Trumpler 14 287  3.97  2733  -0028  0.52  6.83
457 Trumpler 15 287  7.55  1853  -0012  0.43  6.93
458 Collind.232 287  3.49  2996  -0027  0.57  6.67
459 Trumpler 16 287  7.78  2673  -0031  0.49  6.79
460 Bochum 11   288 14.73  2412  -0036  0.58  6.76
461 Alessi 5    288  3.82   398  -0014  0.15  7.60
462 Trumpler 17 288  3.18  2189  +0017  0.60  7.71
463 Pismis 17   289  6.12  3504  +0009  0.47  7.02
464 Ruprecht 92 289  4.81  2362  -0082  0.46  7.80
465 N3496       289  2.30   990  -0007  0.47  8.47
466 N3532       289  7.07   486  +0011  0.04  8.49
467 I2602       289  4.68   161  -0014  0.02  7.51
468 Sher 1      289  1.71  5875  -0025  1.37  6.71
469 Bochum 12   289  6.45  2218  -0069  0.24  7.61
470 Melotte 101 289  8.70  1995  -0193  0.48  7.89
471 Feinstein 1 290  8.43  1159  +0008  0.40  7.00
472 Ruprecht 93 290  2.93  1437  -0028  0.23  8.19
473 Stock 13    290  2.29  1577  +0044  0.22  7.22
474 N3572       290  2.90  1995  +0007  0.39  6.89
475 Hogg 10     290  1.55  1776  +0002  0.46  6.78
476 Collind.240 290  9.17  1577  +0005  0.31  7.16
477 Hogg 11     290  1.32  2277  +0005  0.32  7.08
478 Trumpler 18 290  1.98  1358  -0003  0.32  7.19
479 N3590       291  1.44  1651  -0005  0.45  7.23
480 N3603       291  0.53  3634  -0033  1.34  6.84
481 I2714       292  5.04  1238  -0039  0.34  8.54
482 Mamajek 1   292  1.13    97  -0036  0.00  6.90
483 Melotte 105 292  3.21  2208  -0093  0.48  8.32
484 ESO 093-08  293  3.99 13700  -0965  0.64  9.65
485 N3766       294  2.54  1745  -0001  0.18  7.16
486 N3960       294  3.28  2258  +0243  0.30  8.82
487 I2944       294 18.26  1794  -0052  0.32  6.82
488 Stock 14    295  3.75  2146  -0025  0.22  7.06
489 Ruprecht 97 296  1.97  1357  -0012  0.23  8.34
490 N4052       297  3.17  1209  -0019  0.16  8.50
491 Ruprecht 98 297  2.01   494  -0020  0.16  8.51
492 N4103       297  2.85  1632  +0033  0.29  7.39
493 Sauer 4     298  3.24  6190  -0112  1.24  9.18
494 N4337       299  0.57   489  +0039  0.15  8.45
495 N4349       299  3.16  2176  +0032  0.38  8.32
496 Collind.258 299  1.72  1184  +0041  0.16  8.03
497 Hogg 14     300  0.85   969  +0049  0.23  8.10
498 N4439       300  2.08  1785  +0082  0.35  7.91
499 N4463       300  1.07  1050  -0037  0.43  7.50
500 Collind.261 301  5.73  2190  -0211  0.27  9.95
501 N4609       301  1.42  1223  -0003  0.33  7.89
502 Hogg 15     302  1.32  2262  -0010  1.09  6.78
503 N4755       303  5.75  1976  +0086  0.39  7.22
504 N4815       303  4.48  3079  -0113  0.81  8.37
505 BH 144      305  4.08  9354  -0515  0.60  8.83
506 Collind.268 305  2.86  1963  -0149  0.31  8.76
507 Rupr. 107   305  1.26  1442  -0056  0.46  7.48
508 Stock 16    306  1.43  1640  +0002  0.49  6.92
509 Collind.271 307  1.70  1169  -0033  0.29  8.32
510 Basel 18    307  1.94  2226  +0008  0.52  7.59
511 Hogg 16     307  2.77  1585  +0037  0.41  7.05
512 N5138       307  4.04  1986  +0122  0.26  7.99
513 Trumpler 21 307  1.84  1263  -0007  0.20  7.70
514 Collind.272 307  5.95  2045  +0043  0.47  7.23
515 N5168       307  2.07  1777  +0048  0.43  8.00
516 Pismis 18   308  2.61  2240  +0008  0.50  9.08
517 Rupr. 108   308  2.62   901  +0063  0.14  8.42
518 Platais 11  308 12.14   232  -0015  ...   8.30
519 N5281       309  2.26  1108  -0014  0.22  7.15
520 Platais 10  309 23.15   246  +0013  ...   8.00
521 Platais 12  309 14.03   402  -0010  ...   8.30
522 N5316       310  4.95  1215  +0002  0.27  8.20
523 Lynga 1     310  1.99  2283  -0013  0.46  8.01
524 Alessi 6    313  6.10   437  -0042  0.19  8.20
525 Lynga 2     313  2.91  1000  -0008  0.20  8.12
526 Trumpler 22 314  4.41  1516  -0015  0.52  7.95
527 N5617       314  4.46  1533  -0003  0.48  7.92
528 Pismis 19   314  2.09  2400  -0013  1.45  9.00
529 Melotte 227 314  2.44   120  -0061  0.04  8.57
530 N5606       314  1.58  1805  +0031  0.47  7.08
531 Hogg 17     314  1.52  1310  -0021  0.59  8.03
532 N5460       315  6.90   678  +0148  0.09  8.21
533 N5662       316  5.62   666  +0039  0.31  7.97
534 N5749       319  3.00  1031  +0082  0.38  7.73
535 Pismis 20   320  2.35  2018  -0042  1.18  6.86
536 Hogg 18     320  2.23  1535  +0172  0.50  7.76
537 N5823       321  4.16  1192  +0051  0.09  8.90
538 N5822       321  9.34   917  +0057  0.15  8.82
539 N6025       324  3.08   756  -0078  0.16  7.89
540 N6005       325  3.91  2690  -0140  0.45  9.08
541 N5999       326  1.79  2050  -0069  0.45  8.60
542 Alessi 8    326  4.02   575  +0043  0.09  8.15
543 Loden 2326  327  0.42   900  +0031  0.41  8.30
544 N6087       327  3.63   891  -0084  0.18  7.98
545 BH 176      328 11.69 13400  +1008  0.77  ...
546 Moffat 1    328  6.72  3300  -0057  1.84  6.60
547 N6031       329  1.59  1823  -0048  0.37  8.07
548 N6067       329  5.77  1417  -0055  0.38  8.08
549 Harvard 10  329  9.54  1312  -0075  0.36  8.34
550 Lynga 6     330  2.33  1600  +0009  1.25  7.43
551 Rupr. 115   330  3.14  2160  -0032  0.65  8.78
552 Pismis 22   331  1.16  1000  -0010  2.00  7.60
553 Rupr. 118   332  1.17  1343  -0042  0.41  8.11
554 Rupr. 119   333  2.22   956  -0031  0.57  6.85
555 N6208       333  4.92   939  -0094  0.21  9.07
556 Pismis 23   334  0.76  2600  +0020  2.00  8.48
557 N6134       334  1.59   913  -0003  0.40  8.97
558 N6167       335  2.26  1108  -0028  0.78  7.89
559 N6253       335  1.76  1510  -0164  0.20  9.70
560 Rupr. 120   336  1.75  2000  -0017  0.70  8.18
561 N6193       336  4.70  1155  -0032  0.48  6.78
562 N6200       337  8.36  2054  -0038  0.58  6.93
563 N6178       338  1.47  1014  +0021  0.22  7.25
564 N6204       338  1.58  1085  -0020  0.43  7.56
565 Hogg 22     338  1.06  1216  -0024  0.65  6.78
566 Westerl. 1  339  4.54  5200  -0050  3.00  ...
567 I4651       340  2.58   888  -0122  0.12  9.06
568 N6192       340  4.05  1547  +0057  0.64  8.13
569 N6216       340  5.00  4300  +0000  0.45  7.54
570 N6250       340  2.52   865  +0029  0.35  7.42
571 N6124       340  5.81   512  +0054  0.75  8.15
572 Lynga 14    340  0.77   881  -0017  1.43  6.71
573 N6249       341  1.43   981  -0020  0.44  7.39
574 N6259       341  4.20  1031  -0027  0.50  8.34
575 N6231       343  5.06  1243  +0026  0.44  6.84
576 Alessi 9    344  6.24   195  -0030  0.07  8.40
577 Trumpler 24 344 19.86  1138  +0030  0.42  6.92
578 N6322       345  1.45   996  -0053  0.59  7.06
579 N6242       345  2.96  1131  +0049  0.38  7.61
580 N6268       346  1.80  1029  +0023  0.39  7.24
581 N6281       347  1.11   479  +0016  0.15  8.50
582 N6318       347  2.68  2300  -0028  1.20  6.30
583 Havlen-M 1  348  4.22  2900  -0039  1.85  ...
584 BH 222      349  3.49  6000  -0046  1.85  7.78
585 Bochum 13   351  4.39  1077  +0026  0.85  6.82
586 Rupr. 127   352  2.13  1466  -0064  0.99  7.35
587 Pismis 24   353  2.90  1995  +0022  1.72  7.00
588 N6396       353  1.04  1192  -0037  0.93  7.51
589 Trumpler 27 355  2.11  1211  -0016  1.19  7.06
590 N6383       355  5.73   985  +0001  0.30  6.96
591 N6475       355  7.00   301  -0024  0.10  8.48
592 Trumpler 28 356  1.95  1343  -0007  0.73  7.29
593 N6405       356  2.83   487  -0007  0.14  7.97
594 N6416       356  3.02   741  -0020  0.25  8.09
595 N6425       357  2.26   778  -0022  0.40  7.35
596 Rupr. 130   359  1.83  2100  -0035  1.20  7.70
597 BH 245      359  0.29  1000  -0009  2.25  7.17
598 N6451       359  4.24  2080  -0058  0.67  8.13
599 Collind.347 359  4.40  1514  -0009  1.16  7.08
600 Basel 5     359  1.11   766  -0025  0.32  8.87


